Kimera2: Robust and Accurate Metric-Semantic SLAM in the Real World

We present improvements to Kimera, an open-source metric-semantic visual-inertial SLAM library. In particular, we enhance Kimera-VIO, the visual-inertial odometry pipeline powering Kimera, to support better feature tracking, more efficient keyframe selection, and various input modalities (eg monocular, stereo, and RGB-D images, as well as wheel odometry). Additionally, Kimera-RPGO and Kimera-PGMO, Kimera's pose-graph optimization backends, are updated to support modern outlier rejection methods - specifically, Graduated-Non-Convexity - for improved robustness to spurious loop closures. These new features are evaluated extensively on a variety of simulated and real robotic platforms, including drones, quadrupeds, wheeled robots, and simulated self-driving cars. We present comparisons against several state-of-the-art visual-inertial SLAM pipelines and discuss strengths and weaknesses of the new release of Kimera. The newly added features have been released open-source at https://github.com/MIT-SPARK/Kimera.

==> figures/figure_carsim_dataset.tex <==
%!TEX root = ../../main.tex

\begin{figure}[h]
	% \vspace{-6mm}
	\centering
	\begin{subfigure}[b]{0.5\columnwidth}
		\centering
		\includegraphics[width=\columnwidth]{figures/img/carsim-sample.png}
		\caption{}
		\label{fig:carsim-imgs}
	\end{subfigure}%
	% \hfill
    \begin{subfigure}[b]{0.5\columnwidth}
		\centering
		\includegraphics[width=0.4\columnwidth]{figures/img/sim_0_traj.png}
		\includegraphics[width=0.4\columnwidth]{figures/img/sim_1_traj.png}

		\includegraphics[width=0.4\columnwidth]{figures/img/sim_2_traj.png}
		\includegraphics[width=0.4\columnwidth]{figures/img/sim_3_traj.png}
		\caption{}
		\label{fig:carsim-trajectories}
	\end{subfigure}
	\caption{
		Car-sim datasets, collected in a simluation environment. 
        \ref{fig:carsim-imgs} shows a third-person POV of the car model in a large urban environment developed in the TESSE simulator. 
        The car has a realistic dynamics model. 
        \ref{fig:carsim-trajectories} shows the ground-truth trajectories of the four Car-sim datasets. 
		These datasets were also used in Chapter~\ref{chap:ford}. 
	}
	\label{fig:carsim-dataset}
	% \vspace{-5mm}
\end{figure}


==> figures/figure_kimeraMulti_dataset.tex <==
%!TEX root = ../../main.tex

\begin{figure}[h]
	% \vspace{-6mm}
	\centering
	\begin{subfigure}[b]{0.25\columnwidth}
		\centering
		\includegraphics[width=0.98\columnwidth]{figures/img/jackal.jpg}
		\caption{}
		\label{fig:kimeraMulti-jackal}
	\end{subfigure}%
    \begin{subfigure}[b]{0.25\columnwidth}
        \centering
        \includegraphics[width=0.98\columnwidth]{figures/img/a1.jpg}
        \caption{}
        \label{fig:kimeraMulti-a1}
    \end{subfigure}%
	% \hfill
    \begin{subfigure}[b]{0.5\columnwidth}
		\centering
		\includegraphics[width=0.45\columnwidth]{figures/img/a1_floor6_traj.png}
		\includegraphics[width=0.45\columnwidth]{figures/img/jackal_1014_acl2_traj.png}

		\includegraphics[width=0.45\columnwidth]{figures/img/jackal_1207_acl2_traj.png}
		\includegraphics[width=0.45\columnwidth]{figures/img/jackal_1208_spark2_traj.png}
		\caption{}
		\label{fig:kimeraMulti-trajectories}
	\end{subfigure}
	\caption{
		KimeraMulti datasets, from the A1 and Jackal robots. 
        \ref{fig:kimeraMulti-jackal} shows the Clearpath Robotics Jackal, and \ref{fig:kimeraMulti-a1} is the Unitree A1. 
        \ref{fig:kimeraMulti-trajectories} shows the ground-truth trajectories of four sequences from this dataset.  
	}
	\label{fig:kimeraMulti-dataset}
	% \vspace{-5mm}
\end{figure}


==> figures/figure_uHumans2_dataset.tex <==
%!TEX root = ../../main.tex

\begin{figure}[h]
	% \vspace{-6mm}
	\centering
	\begin{subfigure}[b]{\columnwidth}
		\centering
		\includegraphics[width=\columnwidth]{figures/img/uHumans2_datasets_samples.png}
		\caption{Four simulation environments used in the uHumans2 datasets.}
		\label{fig:uH2-imgs}
	\end{subfigure}
	\hfill
    \begin{subfigure}[b]{\columnwidth}
		\centering
		\includegraphics[width=0.33\columnwidth]{figures/img/uh2_apartment_traj.png}%
		\includegraphics[width=0.33\columnwidth]{figures/img/uh2_office_orig_traj.png}%
		\includegraphics[width=0.33\columnwidth]{figures/img/uh2_subway_traj.png}%
		\caption{Sample ground truth trajectories, not to scale.}
		\label{fig:uH2-trajectories}
	\end{subfigure}
	\caption{
		uHumans2 datasets. 
        Collected in a simulation environment developed for the original Kimera release~\cite{Rosinol20icra-Kimera}. 
        The datasets have been released to the community, and the simulator code is open-source.
		\ref{fig:uH2-imgs} shows snapshots of the four simulation environments used, and~\ref{fig:uH2-trajectories} shows some of the ground-truth trajectories from this dataset. 
	}
	\label{fig:uH2-dataset}
	% \vspace{-5mm}
\end{figure}


==> preamble_algo.tex <==
%!TEX root = main.tex
\lstdefinelanguage{mine} 
{morekeywords={while,True,if,break,=,return,function,for,until,in,input,output,assumptions,assumption,invariant,loop,variant,end,invariant,precondition,variables}, 
sensitive=false, 
morecomment=[l]{\#}, 
morecomment=[il]\%{.}, 
morecomment=[s]{/*}{*/}, 
morestring=[b]", 
} 

\lstset{% general command to set parameter(s) 
basicstyle=\small\rmfamily, % print whole listing small 
keywordstyle=\color{black}\bfseries, 
% underlined bold black keywords 
identifierstyle=, % nothing happens 
commentstyle=\color[rgb]{0.2,0.2,0.2},
stringstyle=\ttfamily, % typewriter type for strings 
showstringspaces=false,
mathescape=true,
fontadjust=true,
columns=fullflexible} % no special string spaces 
\lstset{frameround=fttt,frame=none}

\usepackage{calc}
\newlength\listingnumberwidth
\setlength\listingnumberwidth{\widthof{00}}
\lstset{
numbers=left,
xleftmargin=\listingnumberwidth,
numbersep=1em
}


\lstset{escapeinside={*@}{@*}}

\newcommand{\tuple}[2]{\langle#1,#2\rangle}
